Detecting fake review buyers using network structure: Direct evidence from Amazon

Online reviews significantly impact consumers' decision-making process and firms' economic outcomes and are widely seen as crucial to the success of online markets. Firms, therefore, have a strong incentive to manipulate ratings using fake reviews. This presents a problem that academic researchers have tried to solve over two decades and on which platforms expend a large amount of resources. Nevertheless, the prevalence of fake reviews is arguably higher than ever. To combat this, we collect a dataset of reviews for thousands of Amazon products and develop a general and highly accurate method for detecting fake reviews. A unique difference between previous datasets and ours is that we directly observe which sellers buy fake reviews. Thus, while prior research has trained models using lab-generated reviews or proxies for fake reviews, we are able to train a model using actual fake reviews. We show that products that buy fake reviews are highly clustered in the product-reviewer network. Therefore, features constructed from this network are highly predictive of which products buy fake reviews. We show that our network-based approach is also successful at detecting fake reviews even without ground truth data, as unsupervised clustering methods can accurately identify fake review buyers by identifying clusters of products that are closely connected in the network. While text or metadata can be manipulated to evade detection, network-based features are more costly to manipulate because these features result directly from the inherent limitations of buying reviews from online review marketplaces, making our detection approach more robust to manipulation.

==> RF_classification_results.tex <==

\begin{table}[ht]
\centering
\caption{Out-of-sample prediction performance of the random forests classifier with varying sets of features.}\label{tab:RF_pred_results}
\begin{tabular}{lccccc}
    \hline
    Features&	AUC&Accuracy	&TNR&	TPR&	F1 Score\\
    \hline
    \hline
    Network&\textbf{	.890} &	.\textbf{821} &	.839 &	\textbf{.797} &	\textbf{.821}\\
    Top-2 Network&	.879 &	.812 &	.832 &	.787 &	.812\\
    % Metadata&	.868 &	.791 &	.834 &	.734 &	.791\\
    Metadata&	.874 &	.811 &	.858 &	.748 &	.810\\ % after adding "stdev review len" feature
    Text&	.857 &	.770 &	\textbf{.929} &	.559 &	.759\\
    Image&	.592 &	.599 &	.792 &	.343 &	.577\\
    \hline
    % All Features&	.933 &	.859 &	.879 &	.832 &	.859\\
    All Features&	.932 &	.860 &	.881 &	.832 &	.860\\ % after adding "stdev review len" feature
    \hline
\end{tabular}
\end{table}

==> features_description.tex <==
\begin{table}[ht]
\centering
\small
\caption{Product-level features generated from review content and product network.}\label{tab:features_desc}
\resizebox{\linewidth}{!}{\begin{tabular}{c|l|l}
    \hline
    Type & Feature & Description\\
    \hline
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Network}} 
     & degree & Total number of reviewers in common with other products\\
     & clustering coef & Clustering coefficient of the product\\
     & eigenvector cent & Eigenvector centrality score of the product\\
     & pagerank & PageRank score of the product\\
    \hline
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Metadata}} 
     & tf-idf sim & Avg similarity of TF-IDF features b/w reviews of a product \\
     & \# reviews & Number of reviews\\
     & avg review rating & Avg review ratings \\
     & time b/w reviews & Avg, min, max, and stdev of time in days b/w reviews\\
     %& avg days between reviews & Average time in days between reviews \\
     %& std days between reviews & Stdev. of time in days between reviews\\
     %& max days between reviews & Maximum time in days between reviews \\
     %& min days between reviews & Minimum time in days between reviews\\
     & share helpful & Share of reviews with helpful votes\\
     & share 1star & Share of reviews with 1-star rating\\
     & share 5star & Share of reviews with 5-star rating\\
     & share photo & Share of reviews with review photo\\
     & stdev review len & Variation of review lengths of a product\\
    \hline
    \multirow{3}{*}{\rotatebox[origin=c]{90}{Image}} 
    & img sim& Avg, min, max, and stdev of image similarity b/w product reviews \\
    & sim review & Avg, min, max, and stdev of similarity b/w all pairs of review images \\
    & sim product& Avg, min, max, and stdev of similarity b/w product and review images \\
    %  & min sim & Minimum pair-wise similarity \\
    %  & max sim & Maximum pair-wise similarity  \\
    %  & avg sim & Average pair-wise similarity  \\
    %  & std sim & Stdev. of all pair-wise similarities  \\
    %  & min sim review & Minimum pair-wise similarity between review images\\ 
    %  & max sim review & Maximum pair-wise similarity between review images \\
    %  & avg sim review & Average pair-wise similarity between review images \\
    %  & std sim review & Stdev. of all pair-wise similarities between review images\\
    % & min sim product & Minimum pair-wise similarity between review and product images\\
    % & max sim product & Maximum pair-wise similarity between review and product images\\
    % & avg sim product & Average pair-wise similarity between review and product images\\
    % & std sim product & Stdev. of pair-wise similarities between review and product images\\
    \hline
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Text}} &\multirow{2}{*}{tf-idf} &\multirow{2}{*}{Top 1000 TF-IDF features of a product} \\
    & & \\
    \hline
\end{tabular}}
\end{table}

==> tables/RF_classification_results.tex <==

\begin{table}[ht]
\centering
\caption{Out-of-sample prediction performance of the random forests classifier with varying sets of features.}\label{tab:RF_pred_results}
\begin{tabular}{lccccc}
    \hline
    Features&	AUC&Accuracy	&TNR&	TPR&	F1 Score\\
    \hline
    \hline
    Network&\textbf{	.890} &	.\textbf{821} &	.839 &	\textbf{.797} &	\textbf{.821}\\
    Top-2 Network&	.879 &	.812 &	.832 &	.787 &	.812\\
    % Metadata&	.868 &	.791 &	.834 &	.734 &	.791\\
    Metadata&	.874 &	.811 &	.858 &	.748 &	.810\\ % after adding "stdev review len" feature
    Text&	.857 &	.770 &	\textbf{.929} &	.559 &	.759\\
    Image&	.592 &	.599 &	.792 &	.343 &	.577\\
    \hline
    % All Features&	.933 &	.859 &	.879 &	.832 &	.859\\
    All Features&	.932 &	.860 &	.881 &	.832 &	.860\\ % after adding "stdev review len" feature
    \hline
\end{tabular}
\end{table}

==> tables/features_description.tex <==
\begin{table}[ht]
\centering
\small
\caption{Product-level features generated from review content and product network.}\label{tab:features_desc}
\resizebox{\linewidth}{!}{\begin{tabular}{c|l|l}
    \hline
    Type & Feature & Description\\
    \hline
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Network}} 
     & degree & Total number of reviewers in common with other products\\
     & clustering coef & Clustering coefficient of the product\\
     & eigenvector cent & Eigenvector centrality score of the product\\
     & pagerank & PageRank score of the product\\
    \hline
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Metadata}} 
     & tf-idf sim & Avg similarity of TF-IDF features b/w reviews of a product \\
     & \# reviews & Number of reviews\\
     & avg review rating & Avg review ratings \\
     & time b/w reviews & Avg, min, max, and stdev of time in days b/w reviews\\
     %& avg days between reviews & Average time in days between reviews \\
     %& std days between reviews & Stdev. of time in days between reviews\\
     %& max days between reviews & Maximum time in days between reviews \\
     %& min days between reviews & Minimum time in days between reviews\\
     & share helpful & Share of reviews with helpful votes\\
     & share 1star & Share of reviews with 1-star rating\\
     & share 5star & Share of reviews with 5-star rating\\
     & share photo & Share of reviews with review photo\\
     & stdev review len & Variation of review lengths of a product\\
    \hline
    \multirow{3}{*}{\rotatebox[origin=c]{90}{Image}} 
    & img sim& Avg, min, max, and stdev of image similarity b/w product reviews \\
    & sim review & Avg, min, max, and stdev of similarity b/w all pairs of review images \\
    & sim product& Avg, min, max, and stdev of similarity b/w product and review images \\
    %  & min sim & Minimum pair-wise similarity \\
    %  & max sim & Maximum pair-wise similarity  \\
    %  & avg sim & Average pair-wise similarity  \\
    %  & std sim & Stdev. of all pair-wise similarities  \\
    %  & min sim review & Minimum pair-wise similarity between review images\\ 
    %  & max sim review & Maximum pair-wise similarity between review images \\
    %  & avg sim review & Average pair-wise similarity between review images \\
    %  & std sim review & Stdev. of all pair-wise similarities between review images\\
    % & min sim product & Minimum pair-wise similarity between review and product images\\
    % & max sim product & Maximum pair-wise similarity between review and product images\\
    % & avg sim product & Average pair-wise similarity between review and product images\\
    % & std sim product & Stdev. of pair-wise similarities between review and product images\\
    \hline
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Text}} &\multirow{2}{*}{tf-idf} &\multirow{2}{*}{Top 1000 TF-IDF features of a product} \\
    & & \\
    \hline
\end{tabular}}
\end{table}
